WKB and Turning Point Theory for Second Order Difference Equations: External Fields and Strong Asymptotics for Orthogonal Polynomials

A LG-WKB and Turning point theory is developed for three term recurrence formulas associated with monotonic recurrence coefficients. This is used to find strong asymptotics for certain classical orthogonal polynomials including Wilson polynomials.

==> references.tex <==
\bibitem{AGV} { A. I. Aptekarev, J. S  Geronimo, and W. Van Assche},
              {Varying weights for orthogonal polynomials with monotonically
              varying recurrence coefficients},
              {\it J. Approx. Theory, \bf 150}, {2008}, {214--238}.

\bibitem{BKMM} {J. Biak, T. Kriecherbauer, K. T.-R. Mclaughlin and
              P.D. Miller}, {Discrete orthogonal polynomials}, {Annals of
              Mathematics Studies}, {Princeton University Press}, {Princeton,
              NJ}, {2007}.

\bibitem{BI}{P. Bleher and A. Its},
{Semiclassical asymptotics of orthogonal polynomials,
              {R}iemann-{H}ilbert problem, and universality in the matrix
              model},
{\it Ann. of Math. (2), \bf 150}, {1999}, {185--266}.


\bibitem{BR} {V. S. Buyarov and E. A. Rakhmanov},
     {On families of measures that are balanced in the external
     field on the real axis},
   {\it Mat. Sb.}
%  {\it Rossi\u\i skaya Akademiya Nauk. Matematicheski\u\i\ Sbornik},
    {\bf 190}, \#6
      {(1999)},
     {11--22}.

\bibitem{CI}{Y. Chen,  and M. E. H Ismail}, {Asymptotics of extreme zeros of
      the {M}eixner-{P}ollaczek polynomials}, {\it
      J. Comput. Appl. Math. \bf 82},  {(1997)}, {59--78}.


\bibitem{C} T. S. Chihara,  An introduction to orthogonal polynomials, 
Mathematics and its Applications, Vol. 13. Gordon and Breach Science Publishers, 
New York-London-Paris, 1978.

\bibitem{CC} O. Costin, R. Costin, Rigorous WKB method for finite-order
linear recurrence relations with smooth coefficients, {\it SIAM J. Math.
Anal. \bf 27} (1996) 110--134.

\bibitem{Do}{D. Dominici},
{Asymptotic analysis of the {K}rawtchouk polynomials by the {WKB} method},
{\it Ramanujan J. \bf 15}, {(2008)}, {303--338}.


\bibitem{DS} {P. D. Dragnev and E. B. Saff},
     {Constrained energy problems with applications to orthogonal
     polynomials of a discrete variable},
   {\it J. Anal. Math.}
%  {\it Journal d'Analyse Math\'ematique},
    {\bf 72}, {(1997)}, {223--259}.


\bibitem{DKMVZ} {P. Deift, T. Kriecherbauer, K. T-R. McLaughlin,
              S. Venakides, and X. Zhou},
     {Strong asymptotics of orthogonal polynomials with respect to
     exponential weights},
   {\it Comm. Pure Appl. Math.},
%  {Communications on Pure and Applied Mathematics},
    {\bf 52}, \#12
      {(1999)},
     {1491--1552}.

\bibitem{DM} P. Deift, K. T-R. McLaughlin, A Continuum Limit of
the Toda Lattice, {\it Memoirs of AMS \bf \#624} (1998) Providence, RI.

\bibitem{FW} C. L. Frenzen and R. Wong, Uniform asymptotic expansions of
Laguerre polynomials.  {SIAM. J. Math. Anal.} {\bf 19}  (1988), 1232--1248.

\bibitem{GG} {S. Garoufalidis and J. S. Geronimo},
             {Asymptotics of {$q$}-difference equations},
             {Primes and knots}, {\it Contemp. Math. \bf 416}, {83--114},
             {Amer. Math. Soc.}, {Providence, RI}, {2006}.


\bibitem{GBVA} J. S. Geronimo, O. Bruno, and W. Van Assche,
     {WKB and turning point theory for second-order difference
     equations}, in
 {\it Spectral Methods for Operators of Mathematical Physics},
    {Oper. Theory Adv. Appl.},
     {\bf 154},
     {101--138},
 {Birkh\"auser}, {Basel},
      {(2004)}.


\bibitem{GBVAe} {J. S. Geronimo, O. Bruno, and W. Van Assche},
     {WKB and turning point theory for second-order difference
     equations} {errata}.

\bibitem{GS}{J. S. Geronimo, and D. Smith,} WKB (Liouville-Green) Analysis of
Second Order Difference Equations and Applications, {\it JAT \bf 69}
(1992) 269--301.

\bibitem{GSV}{J. S. Geronimo, D. Smith, and W. Van Assche},
{Strong asymptotics for orthogonal polynomials with regularly
              and slowly varying recurrence coefficients},
{\it J. Approx. Theory, \bf 72},
{1993},
{141--158}.

\bibitem{GVA} J. S. Geronimo  and W. Van Assche, {Relative asymptotics
for orthogonal polynomials with unbounded recurrence coefficients},
JAT, {\bf 62}, {(1990)}, 47--69.


\bibitem{GR} {A. A. Gonchar and E. A. Rakhmanov},
     {The equilibrium measure and distribution of zeros of extremal
     polynomials}, Mat. Sb. (N.S.),
%  FJOURNAL = {Matematicheski\u\i\ Sbornik. Novaya Seriya},
    {\bf 125}(167) \#1(9)
      {(1984)},
     {117--127}.

\bibitem{JN}{J. Janas and S. Naboko}, {Jacobi Matrices with Power-like
Weights--Grouping in Blocks approach}, {\it J. Funct. Anal. \bf 166}, {(1999)},
{218--243}.

\bibitem{JWa} X-S Jin and R. Wong, {Uniform asymptotic expansions for Meixner
      polynomials},  {\it \hbox{Constr.} Approx. \bf 14}  (1998),  113--150.

\bibitem{JWb} X-S. Jin, and R. Wong, {Asymptotic formulas for the zeros of
the Meixner polynomials},  JAT. {\bf 96}  (1999), 281--300.

\bibitem{KS} R. Koekoek and R. F. Swarttouw, {The Askey-scheme of 
hypergeometric orthogonal polynomials and its $q$-analogue}, 
Report No. 98--17, Delft Univ. Tech. (1998).

\bibitem{KM} {T. Kriecherbauer and K. T.-R. McLaughlin},
     {Strong asymptotics of polynomials orthogonal with respect to
     Freud weights},
   {\it Internat. Math. Res. Notices \bf 6},
%%  FJOURNAL = {International Mathematics Research Notices},
      {(1999)},
     {299--333}.

\bibitem{KR} {A. B. J. Kuijlaars and E. A. Rakhmanov},
     {Zero distributions for discrete orthogonal polynomials},
 in {\it Proceedings of the VIIIth Symposium on Orthogonal Polynomials
        and Their Applications} (Seville, 1997),
   {\it J. Comput. Appl. Math.}
%%  FJOURNAL = {Journal of Computational and Applied Mathematics},
    {\bf 99}, \#1--2
      {(1998)},
     {255--274}.

\bibitem{KVA} {A. B. J. Kuijlaars and W. Van Assche},
     {The asymptotic zero distribution of orthogonal polynomials
     with varying recurrence coefficients},
   {\it J. Approx. Theory}
%%  FJOURNAL = {Journal of Approximation Theory},
    {\bf 99}, \#1
      {(1999)}
     {167--197}.

\bibitem{KVAt} {A. B. J. Kuijlaars and W. Van Assche},
     {Extremal polynomials on discrete sets},
{\it Proc. London Math. Soc. \bf 3}, {(1999)}, {191--221},

\bibitem{MV}{M. Maejima and W. Van Assche},
{Probabilistic proofs of asymptotic formulas for some classical
              polynomials},
{\it Math. Proc. Cambridge Philos. Soc.\bf 97}, {1985},
{499--510}.

\bibitem{LLone} {A. L. Levin and D. S. Lubinsky},
     {Green equilibrium measures and representations of an external
     field},
   {\it J. Approx. Theory},
%%  FJOURNAL = {Journal of Approximation Theory},
    {\bf 113}, \#2
      {(2001)}
     {298--323}.

\bibitem{LLtwo} {A. L. Levin and D. S. Lubinsky},
     {Orthogonal polynomials for exponential weights},
    {CMS Books in Mathematics/Ouvrages de Math\'ematiques de la
    SMC, 4},
 {Springer-Verlag},
   {New York},
      {2001}.

\bibitem{LW} X. Li and R. Wong, {On the asymptotics of the Meixner-Pollaczek
    polynomials and their zeros.}  Constr. Approx.  {\bf 17}  (2001),
    59--90.

\bibitem{No}{P. Nevai,}
{Asymptotics for orthogonal polynomials associated with 
{$\exp(-x\sp{4})$}},
{\it SIAM J. Math. Anal. \bf 15},
{1984}, {1177--1187}.

\bibitem{Nt}P. Nevai and
G\'eza {F}reud, Orthogonal polynomials and {C}hristoffel  functions. 
{A} case study,
{\it J. Approx. Theory \bf 48}, {1986}.

\bibitem{ND}{P. G. Nevai and J. Dehesa},
{On asymptotic average properties of zeros of orthogonal polynomials},
{\it SIAMJ. Math. Anal. \bf 10}, {(1979)}, {1184--1192}.

\bibitem{PR}{M. Plancherel and W. Rotach}, {Sur les 
valeurs asymptotiques des polynomes d'Hermite {$H_n(x)=(-1)^n
e^{-{x^2\over2}}/dx^n$},} {\it Comment.Math. Helvet. \bf 1}, {1929}, {227--254}.


\bibitem{O} F. W. J. Olver, {\it Asymptotics and Special Functions}
(1974) Academic Press London.

\bibitem{Raone} {E. A. Rakhmanov},
     {Asymptotic properties of orthogonal polynomials on the real
     axis},
   {\it Mat. Sb. (N.S.)},
%%  FJOURNAL = {Matematicheski\u\i\ Sbornik. Novaya Seriya},
    {\bf 119(161)}, \#2
      {(1982)},
     {163--203, 303}.

%\bibitem{Ratwo} {E. A. Rakhmanov},
%     {Strong asymptotics for orthogonal polynomials},
%in {\it Methods of approximation theory in complex analysis and
%       mathematical physics} (Leningrad, 1991),
%    {\it Lecture Notes in Math.},
%    {\bf 1550},
%     {71--97}.

\bibitem{Rathree} {E. A. Rakhmanov},
        {Equilibrium measure and the distribution of zeros of the extremal
        polynomials of a discrete variable}
       {\it Mat Sb. (N.S.)},
       {\bf 187},
       {(1996)},
       {109--124}.

\bibitem{R}{W. Rudin},
{Real and Complex Analysis 3ed},
{McGraw-Hill}, {1987}.

\bibitem{ST}  {E. B. Saff and V. Totik},
     {Logarithmic potentials with external fields},
    {\it Grundlehren der Mathematischen Wissenschaften [Fundamental
        Principles of Mathematical Sciences]},
    {\bf 316},
      {Appendix B by Thomas Bloom},
 {Springer-Verlag}, {Berlin},
      {1997}.

\bibitem{Sh}{R. C. Sheen},
{Plancherel-Rotach-type asymptotics for orthogonal polynomials with 
 $\exp(-x\sp{6})$}, {\it J. Approx. Theory \bf 50}, {1987}, {232--293}.

\bibitem{SG}{K. Schulten, and R. G. Gordan}, 
{Semiclassical approximations to {$3j$}- and
{$6j$}-coefficients for quantum-mechanical coupling of angular momenta},
{\it J. Mathematical Phys. \bf 16}, {(1975)}, 1971--1988.

\bibitem{S} G. Szeg\"o, {\it Orthogonal Polynomials}, AMS Colloq. Pub.
Vol. 23, 4th ed, Providence, RI (1978).

\bibitem{VG}{W. Van Assche, and J. S. Geronimo}, {Asymptotics for orthogonal
polynomials with regularly varying recurrence coefficients},
{\it Rocky Mtn. J. Math. \bf 19} (1989) 39--49.

\bibitem{V}{W. Van Assche}, {Asymptotics for Orthogonal Polynomials},
{\it Lecture Notes in Mathematics \bf 1265}, {Springer-Verlag}, {Berlin}, {1987}.

\bibitem{VK} {M. Vanlessen and A. B. J. Kuijlaars},
{Strong Asymptotics of Laguerre-type orthogonal polynomials and
applications in random matrix theory}, {arXiv:math CA/0504604 v2}, (2005).

\bibitem{WW} {Z. Wang  and R. Wong},
     {Asymptotic expansions for second-order linear difference
     equations with a turning point},
   {\it Numer. Math.},
%%  FJOURNAL = {Numerische Mathematik},
    {\bf 94}, 
      {(2003)}
     {147--194}.

\bibitem{W} G. N. Watson, {\it A treatise on the theory of Bessel
functions} (2nd ed), Cambridge Univ Press (1944) London.

\end

